On the Error of Random Sampling: Uniformly Distributed Random Points on Parametric Curves

Given a parametric polynomial curve $\gamma:[a,b]\rightarrow \mathbb{R}^n$, how can we sample a random point $\mathfrak{x}\in \mathrm{im}(\gamma)$ in such a way that it is distributed uniformly with respect to the arc-length? Unfortunately, we cannot sample exactly such a point-even assuming we can perform exact arithmetic operations. So we end up with the following question: how does the method we choose affect the quality of the approximate sample we obtain? In practice, there are many answers. However, in theory, there are still gaps in our understanding. In this paper, we address this question from the point of view of complexity theory, providing bounds in terms of the size of the desired error.

==> 2NEWTON.tex <==
We finish with a stronger notion of sample where the error is not only polylogaritmic in the error, but in the number of digits of the error.

\begin{defi}
Given a random variable $\fkx\in \bbR$, a \emph{hyper-efficient sampler for $\fkx$} is a pair of BSS programs $\textsc{S}:\bbN\times \bbR^k\times[0,1]^l\rightarrow \bbR$ and $\textsc{P}:\bbN\rightarrow \bbR^k$ such that: S1) on input $(\ell,u,x)$, the run-time of $\textsc{S}$ is at most $\mathrm{polylog}(\ell)$, S2) on input $\ell$, the run-time of $\textsc{P}$ is at most $\mathrm{poly}(\ell)$, and S3) if $\fku\in[0,1]^l$ is uniformly distributed, then $\fkx_{\ell}:=\textsc{S}(\ell,\textsc{P}(\ell),\fku)$ is a random variable such that
\[
\distTV(\fkx_\ell,\fkx)\leq 2^{-\ell}.
\]
\end{defi}

Note that a hyper-efficient sampler is exponentially faster than an efficient sampler.

\subsection{Assumptions of our analysis \label{sec:assump}}

Let   $\varphi:I\rightarrow \mathbb{R}$ be the density under consideration, for $I$ a real closed interval, and 
\begin{equation}
    \Phi(t):=\int_a^t\,\varphi(s)\,\mathrm{d}s
\end{equation}
the corresponding cumulative distribution function. Our discussion will be based on the following four simplifying assumptions:
\begin{enumerate}
\item[(A0)] $I=[0,1]$.
\item[(A1)] $\varphi$ is positive on $I$.
\item[(A2)] $\varphi'$ is non-negative on $I$.
\item[(A3)] We can compute $\varphi$ and $\Phi$ exactly in the computational model.
\end{enumerate}
These assumption can be justified as follows:
\begin{enumerate}
\item[(A0)] By a linear change of coordinates we can always assume that $I$ is the interval $[0,1]$.
\item[(A1)] In the cases of interest, we express the support of $\varphi$ inside $I$ as a union of intervals. Thus it is enough to perform inverse transform sampling on each one of these intervals.
\item[(A2)] By partitioning $I$ into intervals $J_1,\ldots, J_k$, we can assume that $\varphi'_{|J_k}$ is always non-negative or non-positive. In the latter case, we have to perform a linear change of variables–––of the form $aT+b$ with $a<0$---to force $\varphi'$ to be non-negative. 
\item[(A3)] We will be assuming that we can substitute $\varphi$ by another density $\tilde{\varphi}$ such that both $\tilde{\varphi}$ and
\begin{equation}
    \tilde{\Phi}(t):=\int_0^t\,\tilde{\varphi}(s)\,\mathrm{d}s
\end{equation}
can be computed in the considered computational model. Using Proposition~\ref{prop:TVL1}, we can then guarantee that the obtained random variable is a good approximate sample as long as we can guarantee that the $L^1$-distance between $\varphi$ and $\tilde{\varphi}$ is sufficiently small. The latter is of particular importance to the case under consideration, where will use Chebyshev approximation to approximate $\varphi$. 
\end{enumerate}
Note that the above transformations can also be performed under finite precision, and so in practice. The trick is that the theoretical partition $\{J_k\}$ can be approximated by a partition $\{\tilde{J}_k\}\cup \{E\}$ where a) $\tilde{J}_k\subseteq J_k$ has floating-point endpoints, and b) $\bbP(\fkx\in E)$ small enough, to guarantee that \nameref{alg:partitionsampler} is within the desired limits of precision.

Under the above assumptions, the question is: how does the method used to approximately solve
\begin{equation}\label{eq:invtransequation}
    \Phi(t)=u\in[0,1]
\end{equation}
affect the precision and complexity of inverse transform sampling?

\subsection{Inverse Transform by Newton}

By our assumptions, $\Phi$ is a convex monotone function for which the Newton's method is guaranteed to converge. In pseudocode:

\begin{algorithm}
\DontPrintSemicolon
\SetKwInOut{input}{Input}
\SetKwInOut{output}{Output}
\caption{\textsc{NewtonSampler}}\label{alg:newtonsampler}
\input{$\varphi:[0,1]\rightarrow [0,\infty)$ such that $\int_0^1\varphi(t)\,\mathrm{d}t=1$, $\varphi'\geq 0$\\
$\ell\in\bbN$}
\output{Approximate sample $\fkx$ for $\varphi$}
Sample $\fku\in [0,1]$ uniformly\;
$x\gets 1$\;
$i\gets 0$\;
\While{$i<\ell$}{
$x\gets x+(u-\Phi(x))/\varphi(x)$\;
$i\gets i+1$\;
}
Output $x$\;
\end{algorithm}

Newton's method produces a sequence $\{\Psi_\ell:[0,1]\rightarrow[0,1]\}$ of approximations of $\Phi^{-1}$ given by
\begin{equation}
    \Psi_\ell(u):=\begin{cases}
        1&\text{if }\ell=0,\\
        \Psi_{\ell-1}(u)+\frac{u-\Phi(\Psi_{\ell-1}(u))}{\varphi(\Psi_{\ell-1}(u))}&\text{if }\ell\geq 1,
    \end{cases}
\end{equation}
where $u\in[0,1]$. In this way, \nameref{alg:newtonsampler} gives a sequence $\{\fkx_\ell\}$ of random variables given by
\begin{equation}
    \fkx_\ell:=\Psi_\ell(\fku)
\end{equation}
where $\fku\in[0,1]$ is uniformly distributed. Now, how does $\distTV(\fkx,\fkx_\ell)$ converge to zero? The following lemma gives shows this.

\begin{theo}\label{theo:convergenceTVNewton}
In the above notation. For $\ell\geq 1$,
\begin{equation}
    \distTV(\fkx_\ell,\fkx)\leq \|\Phi\circ \Psi_\ell-1\|_\infty.
\end{equation}
\end{theo}
\begin{lem}\label{lem:inyectivity}
For $\ell\geq 1$, the maps $\Psi_\ell:[0,1]\rightarrow [0,1]$ are monotone, injective and have $1$ as a fixed point.
\end{lem}
\begin{proof}[Proof of Theorem~\ref{theo:convergenceTVNewton}]
By definition of $\fkx_\ell$ and the change of variables theorem, we have that
\[\delta_{\fkx_\ell}(x)=\left(\Psi_\ell'(\Psi^{-1}_\ell(x))\right)^{-1}\chi_{\im \Psi_\ell},\]
where $\chi_{\im \Psi_\ell}$ is the characteristic function of $\im \Psi_\ell$. Therefore for every $B\in \mcB$,
\[|\bbP(\fkx_\ell\in B)-\bbP(\fkx\in B)|=\left|\int_{B\cap \im\Psi_\ell}\left(\Psi_\ell'(\Psi^{-1}_\ell(x))\right)^{-1}-\varphi(x)\,\mathrm{d}x\right|.\]
By the change of variables theorem, using $x=\Psi_\ell(u)$, we obtain
\[|\bbP(\fkx_\ell\in B)-\bbP(\fkx\in B)|=\left|\int_{\Psi^{-1}_\ell(B)}\left(1-\varphi(\Psi_\ell(u))\Psi_\ell'(u)\right)\mathrm{d}x\right|.\]
Hence, for an arbitrary $X\in\mcB$, we have to bound
\[
\left|\int_{X}(\mathrm{id}-\Phi\circ \Psi_\ell)'(u)\,\mathrm{d}x\right|.
\]
If $X=\bigcup_{i=1}^k(a_i,b_i)$, with $a_1<b_1\leq a_2<b_2\leq\ldots$, then 
\[\int_{X}(\mathrm{id}-\Phi\circ \Psi_\ell)'(u)\,\mathrm{d}x=\sum_{i=1}^k(b_i-a_i+\Phi(\Psi_\ell(b_i))-\Phi(\Psi_\ell(a_i))).\]





Note that Lemma~\ref{lem:inyectivity} is needed for using the change of variables as we did.
\end{proof}
\begin{proof}[Proof of Lemma~\ref{lem:inyectivity}]
The claim that $\Psi_\ell(1)=1$ is trivial. Now, if for some $u,v$ and $\ell\geq 1$, we have $\Psi$
\end{proof}

Note that we can easily guarantee that $\Phi\circ\Psi_\ell$ converges uniformly to $1$, but this is not enough! We need this convergence to be also at the level of derivatives.

\subsection[Inverse Transform by off-line Bisection and on-line Newton]{Inverse Transform\\by off-line Bisection and on-line Newton}


\subsection{Inverse Transform by other methods}

Instead of the bisection method, suppose that we use Newton's method. We will have a sequence of approximate solvers
\begin{equation}
    \Psi_\ell(u)=\Psi_{\ell-1}(u)+\frac{u-\Phi(\Psi_{\ell-1}(u))}{\varphi(\Psi_{\ell-1}(u))}
\end{equation}
for $\ell\geq 1$, where $\Psi_0$ is an appropriately chosen continuous function to guarantee that $\{\Psi_\ell\}$ converges to the inverse of $\Phi$.

Let's ignore the issue of choosing $\Psi_0$ and consider that we have a sequence $\{\Psi_\ell\}$ of easily computable functions converging to the inverse of $\Phi$. Under which conditions can we expect $\{\Psi_\ell(\fku)\}$, with $\fku\in[0,1]$ uniformly distributed, to converge to $\fkx$ in the total variation distance? Now, by Proposition~\ref{prop:TVL1}, we have that
\[
\distTV(\Psi_\ell(\fku),\fkx)\leq \|\delta_{\Psi_\ell(\fku)}-\varphi\|_1,
\]
where $\delta_{\Psi_\ell(\fku)}$ is the density function of $\Psi_\ell(\fku)$.
Assuming that the $\Psi_\ell$ is injective, we have, by the change of variables theorem, that
\[
\delta_{\Psi_{\ell}(\fku)}(x)=\frac{\chi_{\Psi_{\ell}[0,1]}(x)}{|\Psi_{\ell}'(\Psi^{-1}(x))|}
\]
where $\chi_{\Psi_{\ell}[0,1]}$ is the characteristic function of $\Psi_\ell[0,1]$. Hence, we need that
\[
\left\|\frac{\chi_{\Psi_\ell[0,1]}(x)}{|\Psi_\ell'(\Psi^{-1}(x))|}-\varphi\right\|_1\to 0,
\]
or equivalently, using a change of variables, that
\[
\|1-(\Phi\circ \Psi_\ell)'\|_1=\|1-(\varphi\circ \Psi_\ell)\Psi_\ell'\|_1\to 0.
\]
Therefore, the problem lies in the fact that even if $u-\Phi\circ\Phi_\ell(u)$ converges uniformly to zero, this convergence does not guarantee that we have $L^1$-convergence of the derivative. This motivates the following question:

\begin{question}
Under which conditions and for which method producing a sequence of approximations $\{\Psi_\ell\}$ of the inverse of $\Phi:[a,b]\rightarrow [0,1]$ can we guarantee that $\Phi\circ \Psi_\ell$ converges to the identity not only uniformly but also at the level of the derivatives?
\end{question}

Answering the above question lies at the center of measuring the error of using Newton's method for inverse transform sampling.

==> 3OLDINTRO.tex <==
\section{Introduction}

Given a parametric polynomial curve $\gamma: I:=[a,b]\rightarrow \bbR^n$, we are interested in \modif{generating a random} point $\fkx\in I$ so that $\gamma(\fkx)$ is uniformly distributed in the curve $\gamma(I)$ (with respect the arc-length). To do this, we only need to sample $\fkt\in I$ with density proportional to the \modif{normalized} speed of the curve $\norm{\gamma'}_2$. Even if we perform exact arithmetic operations and operate with real numbers with infinite precision, \modif{the problem of sampling $\fkt\in I$ with the aforementioned density cannot be done exactly. In general, the integral of this density cannot be expressed in terms of elementary functions.} The goal of this paper is to estimate how much the generated sample differs from the one that we want and how does the desired error affects complexity.

Sampling from a density is an important and well-studied problem in computational statistics. There are many methods to sample according to a certain distribution: Acceptance-Rejection (AR) method~\cite{Leydold98}, Adaptive Rejection Sampling~\cite{Gilks92}, Slice Sampling~\cite{Neal03}, etc. Currently, the state-of-the-art samplers are the so-called
Markov Chain Monte Carlo (MCMC) algorithms have plenty of success stories, such as Hamiltonian Monte Carlo~\cite{NealMCMC}, Hit-and-Run~\cite{Smith96} and Metropolis-Hastings~\cite{chibgreenberg1995}. However, most of them apply only for log-concave distributions~\cite{lovasz2006hit,Lovasz06,chen2019optimal,lee2018algorithmic,dwivedi2019log}. The algorithm in~\cite{pmlr-v99-mangoubi19a} can be used to sample from (multivariate) non-convex density functions, but it does not handle the case where the density is restricted to an interval (or a bounded set in general). Moreover, for the univariate setting, the existing MCMC algorithms~\cite{Johndrow18} either do not provide any guarantees or could lead to arbitrary high run-times.

The problem of sampling \modif{from an arbitrary density function} is empirically studied in~\cite{Olver13}. They propose a practical method that samples from a (probability) density in one or two variables. Their method efficiently blends inverse transform sampling and Chebyshev approximations. Inverse transform sampling is based on solving the equation
\[
\Phi(\fkx)=\fku
\]
for some uniformly distributed $\fku\in[0,1]$ and the cumulative distribution function $\Phi$ of the considered distribution. If we could solve the equation exactly, then $\fkx$ would have the desired distribution. \modif{However, this is not possible in general, so they employ a Chebyshev polynomials to approximate $\Phi$ fast enough and then apply the bisection method.} However, inexact solutions lead to inexact sampling, and there does not seem to be any references regarding the error incurred in the sampling as a consequence of the considered approximations. We aim at filling this gap.

Sampling from a parameterized curve is a topic of interest. In \cite{PAGANI201832}, they propose a sampling method for a certain family of parameterized curves representation \citep{10.5555/265261} based on a mixed parameterization between the arc-length and the curvature and they evaluate the reconstruction performance of their method. 
In \cite{FIGUEIREDO1995173}, the author performs an adaptive method that samples with respect to the local curvature: it consists in recursively performing bisections of the parameter domain and when a parameter interval corresponds to a parametric arc that is almost flat, considering the two endpoints as sample points. 




%In general, describing curves through a parametric representation is common in CAGD and sampling points on curves and surfaces has already received much attention in the literature (see \cite{Surazhsky05samplingplanar,PAGANI201832,10.5555/265261} and references therein); it usually aims in approximating the curve or surface. We can parameterize a curve in various ways, so that uniform sampling of points in its parameter domain, would result in points sampled uniformly according to arc-length, curvature or another density.

%However, in practice, sampling never occurs exactly and none of the previous approaches estimates the quality of the sample, i.e., its deviation from being uniform with respect to a certain density function.

\paragraph{Our contribution}

We provide the first error analysis for sampling points of a polynomial parameterized curve using an algorithm that performs exact arithmetic operations and has a source of randomness. Although our algorithm is similar to that of \cite{Olver13}, our novelty relies on the analysis that establishes a dependence between the desired error and the number of arithmetic operations needed.

%--Say about the sampling method... 
%Our algorithm aims to sample from $\phi(t) \propto \| \gamma'(t) \|,\ t\in [a,b]$, introducing an approximation setting and inverse transform sampling. It generates a sample arbitrarily close to the target distribution w.r.t.\ total variation distance in polynomial time. Our algorithm works in two steps: {\em off-line phase} and {\em on-line phase}. The off-line phase computes an approximation of $\phi(t)$. Our approach is to split the interval $[a,b]$ into proper subintervals $J_i$. Then, we approximate the function $\| \gamma'(t) \|$ with a Chebyshev polynomial $\chevI_{k_{i}}(\| \gamma'(t) \|)$ of degree $k_i$ in each $J_i$. By splitting $[a,b]$ we achieve to reduce the degree of Chebyshev approximation, and thus, speedup our algorithm. Finally, we compute the integrals (normalization factors) of $\chevI_{k_{i}}(\| \gamma'(t) \|),\ t\in J_i$ to obtain the corresponding density functions in each $J_i$ and the weight of each interval. The on-line phase, instead of sampling directly from $\phi(t)$ samples from the piece-wise Chebyshev function defined by $\chevI_{k_{i}}(\| \gamma'(t) \|)$, using the output of the off-line phase. To sample we pick an interval according to its weight. Then we apply inverse transform sampling in that interval, using the density induced by the Chebyshev approximation. We use bisection method to approximate the solution in the step (3) of inverse transform sampling.

\begin{figure}[!t]
	\centering
		\includegraphics[width=0.45\textwidth]{./figures/curve_sampled.png}
	\caption{A parametric polynomial curve of degree $3$ in $\mathbb{R}^3$. From blue to yellow, from smaller to higher values on the z-axis. With red the $10$ points we sampled with our implementation of Alg.~\ref{alg:newsampler}.
	\label{fig:curve_sampled}}
\end{figure}

%We provide several error guarantees. First, we bound the degree of the Chebyshev approximation to achieve an approximation error $\varepsilon$ w.r.t.\ the infinity norm. Then, we integrate this approximation error together with the approximation error of the bisection method to bound the total variation distance between the generated random variable and the target one. We provide complexity bounds for both the preprocess and the online phase of the algorithm. 
We work in the BSS model (see Sec.~\ref{sec:BSS}) for convenience since the approximation of continuous distributions by discrete ones is highly dependent on the application. This model is suitable for developing a complexity theory over the real numbers, since a BSS machine is like a Turing machine, but which can operate with real numbers and perform arithmetic operations and comparisons at cost one.

The main result of this paper is the following one.

\begin{theo}
Let $\gamma :I \rightarrow \mathbb{R}^n$ be a polynomial parameterized curve. The algorithm \nameref{alg:newsampler} samples points from $\gamma$ uniformly with respect to the arc-length by performing
\[
\Oh(\ell^3(1+\log\cond(\gamma))^3\cond(\gamma)^2)
\]
arithmetic operations and with error $2^{-\ell}$ with respect to the total variation distance. $\Oh$ has constants depending on the degree of $\gamma$.
\end{theo}

The technique we employ seems to be quite general, so they open the door to extending our analysis to other continuous random variables in the future. Moreover, this paper is the first one studying reductions of randomness sources in the BSS model of computation.

Moreover, we provide an open-source {\tt Matlab} implementation\footnote{\url{https://github.com/TolisChal/sampling_curves}} of our algorithm. We also provide an extended experimental analysis of the implementation which confirms the theoretical results. We provide efficient computations for all the parameters involved in the pipeline of the algorithm. Our implementation scales up to a few hundred dimensions.

%---(Say that it can be applied to sample wrt to other params...)
%Our algorithm can be applied for sampling with respect to other parameterizations as well. In particular, we believe that our work could extend to other cases of univariate distributions under mild assumptions. We leave this part as a future work. 

\subsection*{Notation}
For a real function $h : I\subseteq \mathbb{R} \rightarrow \mathbb{R}$, its $L^1$ norm is
\begin{equation}
    \|h\|_{1}:=\int_\bbR\,|h(x)|\,ds,
\end{equation}
where, by convention, we take $h(x)=0$ for $x\notin I$.
Its $L^\infty$-norm is defined as $\|h\|_\infty:=\sup_{x\in I}|h(x)|$.

Given a random variable $\fkx\in I$, we will write $\fkx\sim \varphi$ to indicate that $\fkx$ is distributed according to $\varphi$, i.e., $\bbP(\fkx\in J)=\int_{J}\varphi$. We will also denote by $\mcB$ the set of Borel subsets of $\bbR$. 

\subsection*{Organization of the paper}
In Sec.~\ref{sec:efficientsampler} we define the total variation distance of two random variables and introduce the notion of an efficient sampler. In Sec.~\ref{sec:tvdistance} we give bounds on the total variation distance. Inverse transform sampling is illustrated in Sec.~\ref{sec:inv}; we also describe how the univariate solving (that inverse transform sampling requires) is done using the bisection method. A discussion on how the univariate solving can be done using other methods completes this section.
In Sec.~\ref{sec:sampling} we present our curve sampler, study its efficiency and analyze its complexity. We also include a review of Chebyshev approximations. In the end, we present our experimental results~in~Sec.~\ref{sec:implementation}.



